Safe Evaluation For Offline Learning: Are We Ready To Deploy?

The world currently offers an abundance of data in multiple domains, from which we can learn reinforcement learning (RL) policies without further interaction with the environment. RL agents learning offline from such data is possible but deploying them while learning might be dangerous in domains where safety is critical. Therefore, it is essential to find a way to estimate how a newly-learned agent will perform if deployed in the target environment before actually deploying it and without the risk of overestimating its true performance. To achieve this, we introduce a framework for safe evaluation of offline learning using approximate high-confidence off-policy evaluation (HCOPE) to estimate the performance of offline policies during learning. In our setting, we assume a source of data, which we split into a train-set, to learn an offline policy, and a test-set, to estimate a lower-bound on the offline policy using off-policy evaluation with bootstrapping. A lower-bound estimate tells us how good a newly-learned target policy would perform before it is deployed in the real environment, and therefore allows us to decide when to deploy our learned policy.

==> src/pre.tex <==
% \noindent In this section, we introduce reinforcement learning notation and bootstrap confidence intervals.

\subsection{Markov Decision Processes} \label{mdp}
% \josiah{I'm making some edits as I go through but try to follow the guidelines that sets are formatted in caligraphic letters, random variables are capital letters and elements of sets and functions are lower case. You can make exceptions to be consistent with the broader RL literature. If in doubt, check Sutton and Barto notation section.}

We define a control system by a Markov Decision Process or an MDP. An MDP is defined as $(\mathcal{S}, \mathcal{A}, P, r, \gamma, d_0)$, where $\mathcal{S}$ is a set of states, $\mathcal{A}$ is a set of actions, $P$ is a set of probabilities defining the transition from the current states to the next state and $d_0$ is the initial state distribution. An agent acts in an episodic environment by sampling actions from a policy $\pi$ given state $S_t$. 
% \josiah{Not required but you could specify how a trajectory is generated: sample initial state, action, next state and repeat for $L$ time-steps.}
% 
% \josiah{If $L$ is a constant than use lowercase l.} \Hager{it is not constant; it depends on the terminal state, how do i make it clearer?}
A trajectory $H$ of a non-fixed length $L$ is a state-action history, $S_0, A_0, ..., S_{L-1}, A_{L-1}$ where $S_0 \sim d_0, A_t \sim \pi(. | s_t)$ and $S_{t+1} \sim P(.|S_t, A_t)$. The return of a trajectory is $g(H) = \sum_{t=0}^{L-1} \gamma R(S_t, A_t)$ while $v(\pi) := \mathbb{E}_{H \sim \pi} g(H)$ defines the expected discounted return of a policy $\pi$.
% \josiah{Use lower-case $v$ for policy value.}

% \josiah{Need backslash for curly braces in tex. Check elsewhere.}
In the offline learning setup, we define a dataset $\mathcal{D} = \{H_1, H_2, ..., H_n\}$ as a set of $n$ trajectories generated by a behavior policy $\pi_b$. We learn a new policy $\pi_\theta$, the target policy, from $\mathcal{D}$.

% In offline reinforcement learning, we define a data set $D_i$ as a collection of trajectories  of samples where each sample is the state-transition vector: $S_t, A_t, R_t, \gamma_t$ 
% \josiah{I'm confused. Is D transitions or trajectories?}
% \josiah{Again, make sure consistent with what evaluation/target/offline policy is called.}
% \josiah{The HCOPE problem statement is possibly clear enough but could be improved by pointing out that lower bound is a funciton of D which is a random variable. Thus the "with probability" is w.r.t. possible realizations of D.}

\subsection{Bootstrapping}
% \josiah{Going through quickly now but this section needs some work. Not clear what $X$ and $F$ are w.r.t. earlier notation.}
Consider a sample $D$ of $n$ random variables $H_j$ for $j = 1, 2, ..., n$ where we can sample $H_j$ from some $i.i.d$ distribution of data. From the sample of data $D$, we can compute a sample estimate $\hat{\theta}$ of a parameter $\theta$ such  that $\hat{\theta} = f(D)$ where $f$ is the function to compute $\theta$. Given a dataset $D$, we create $B$ resamples with replacement, where $B$ is the number of bootstrap resamples, and compute $\theta$, $\hat{\theta}$, on each of these resamples. Bootstrapping \cite{efron_bootstrap} allows us to estimate the distribution of $\hat{\theta}$ with confidence intervals. The estimates computed with different resamples will be used to determine the 1-$\delta$ confidence interval. In our setup, the parameter of interest $\theta$ is the expected return of a policy $v(\pi)$.

Hence, with a confidence level $\delta \in [0, 1]$ and $B$ resamples of the dataset of trajectories $D$, we use bootstrapping methods to approximate a confidence lower bound of $v_\delta(\pi)$ on $v(\pi)$ such that $v_\delta(\pi) \leq v(\pi)$ with probability at least $1-\delta$. 

As the size of data $n \to \infty$, bootstrapping has strong guarantees but it lacks guarantees for finite samples as it is not an exact method. To use bootstrapping, we have to assume that the bootstrap distribution is representative of the distribution of the static of interest, which is not the case for finite samples \cite{Hanna_MB}. As a result, bootstrapping is considered semi-safe but it is still safe enough for high risk medical predictions in practice with a known record of producing accurate confidence intervals \cite{bootstrap_for_healthcare}.

==> src/results.tex <==
\noindent A case study on when to stop training
